Untangling the nonlinearity in inverse scattering with data-driven reduced order models

The motivation of this work is an inverse problem for the acoustic wave equation, where an array of sensors probes an unknown medium with pulses and measures the scattered waves. The goal of the inversion is to determine from these measurements the structure of the scattering medium, modeled by a spatially varying acoustic impedance function. Many inversion algorithms assume that the mapping from the unknown impedance to the scattered waves is approximately linear. The linearization, known as the Born approximation, is not accurate in strongly scattering media, where the waves undergo multiple reflections before they reach the sensors in the array. Thus, the reconstructions of the impedance have numerous artifacts. The main result of the paper is a novel, linear-algebraic algorithm that uses a reduced order model (ROM) to map the data to those corresponding to the single scattering (Born) model. The ROM construction is based only on the measurements at the sensors in the array. The ROM is a proxy for the wave propagator operator, that propagates the wave in the unknown medium over the duration of the time sampling interval. The output of the algorithm can be input into any off-the-shelf inversion software that incorporates state of the art linear inversion algorithms to reconstruct the unknown acoustic impedance.

==> multidim.tex <==

In this section we generalize the Data to Born transformation from one dimension, 
as described in section \ref{sect:1D}, to multiple dimensions of space $d > 1$.
The derivation follows the same strategy as in section \ref{sect:1D} with 
certain deviations that we emphasize in the discussion below.

%==================================================================================================
\subsection{Data model for an array of sensors}
\label{sect:dataarray}

In the multi-dimensional case we consider an array of $m$ sensors on the 
accessible boundary $\partial \Omega_a$ concentrated at $\bx_s \in \partial \Omega_a$, 
$s = 1,\ldots,m$, each exciting a pressure field
\begin{equation}
\big( \partial_t^2 + A \big) p_s(t, \bx) = \partial_t f(t) \delta(\bx-\bx_s),
\quad - \infty < t < \infty, ~ ~ \bx \in \Omega,
\label{eq:multiwaveps}
\end{equation}
where the operator $A$ is now defined as
\begin{equation}
A = - \sigma(\bx) c(\bx) \nabla \cdot \Big[ \frac{c(\bx)}{\sigma(\bx)} \nabla \Big].
\label{eq:multiA}
\end{equation}
Note that here we assume for simplicity that each sensor emits the same pulse $\partial_t f(t)$.

The boundary conditions are 
\begin{equation}
\nabla p_s(t,\bx) \cdot \bn(\bx) = 0, \quad \bx \in \partial \Omega_a,
\label{eq:multibca}
\end{equation}
where $\bn(\bx)$ is the outer unit normal, and
\begin{equation}
p_s(t,\bx) = 0, \quad \bx \in \partial \Omega_i.
\label{eq:multibci}
\end{equation}
The medium is at rest initially, thus
\begin{equation}
\lim_{t \to -\infty} p_s(t, \bx) = 0, \quad \bx \in \Omega.
\end{equation}

Following the same argument as in \eqref{eq:1D8}--\eqref{eq:1D11} from section 
\ref{sect:1D.1}, we define the matrix-valued data $\bD_k \in \mathbb{R}^{m \times m}$,
$k = 0,\ldots,2n-1$ in terms of its entries
\begin{equation}
(\bD_k)_{i,j} = p_i(t_k, \bx_j) + p_i(-t_k, \bx_j), \quad i,j = 1,\ldots,m,
\end{equation}
where the measurement instances are $t_k = k \tau$ as in the one-dimensional case.
Note that for each $k$ the data matrix $\bD_k$ is symmetric due to the source-receiver
reciprocity.

%==================================================================================================
\subsection{First order form and Liouville transformation}
\label{sect:multifo}

Similarly to the one-dimensional case we introduce the sensor functions
\begin{equation}
b_s(\bx) = \sqrt{\frac{\sigma(\bx_s) c(\bx_s)}{\sigma(\bx)}} 
[\hat f(\sqrt{A})]^{1/2} \delta(\bx - \bx_s), 
\quad \bx \in \Omega, \quad s = 1,\ldots,m.
\end{equation}
and the first order system
\begin{align}
\partial_t \begin{pmatrix} \mathfrak{p}_s(t,\bx) \\ -\mathfrak{u}_s(t, \bx) \end{pmatrix} = 
\begin{pmatrix} 0 & \sigma(\bx) c(\bx) \nabla \cdot \\
\frac{c(\bx)}{\sigma(\bx)} \nabla & 0 \end{pmatrix} \begin{pmatrix}
  \mathfrak{p}_s(t,\bx) \\-\mathfrak{u}_s(t,\bx) \end{pmatrix},
\quad t > 0, \quad \bx \in \Omega,
\label{eq:multifo1}
\end{align}
an analogue of \eqref{eq:1D15} solved by
\begin{equation}
\mathfrak{p}_s(t,\bx) = \cos(t \sqrt{A}) \sqrt{\sigma(\bx)} b_s(\bx), \quad s=1,\ldots,m,
\label{eq:multipfrakcos}
\end{equation}
provided that the initial conditions
\begin{equation}
\mathfrak{p}_s(0,\bx) = \sqrt{\sigma(\bx)} \cb_s(\bx), \quad \mathfrak{u}_s(0,\bx) = 0, 
\quad \bx \in \Omega,
\label{eq:multifo1ic}
\end{equation}
and boundary conditions
\begin{equation}
\mathfrak{p}_s(t,\bx)|_{\bx \in \Omega_i} = 0, \quad 
\mathfrak{u}_s(t,\bx)|_{\bx \in \Omega_a} = 0, \quad t>0,
\label{eq:multifo1bc}
\end{equation}
are imposed.

With the help of Liouville transformation 
\begin{equation}
\cp_s(t,\bx) = \frac{\mathfrak{p}_s(t,\bx)}{\sqrt{\sigma(\bx)}}, \quad 
\cu_s(t,\bx) = -\sqrt{\sigma(\bx)} \mathfrak{u}_s(t,\bx),
\label{eq:multicpcu}
\end{equation}
we can rewrite \eqref{eq:multifo1} as a Schr\"{o}dinger system \eqref{eq:in.1} 
with the operators $L_q$ and $L_q^T$ given by
\begin{align}
L_q   & = - c(\bx) \nabla \cdot \; + \frac{1}{2} c(\bx) \nabla q(\bx) \; \cdot \;, 
\label{eq:multilq} \\
L_q^T & = c(\bx) \nabla + \frac{1}{2} c(\bx) \nabla q(\bx),
\label{eq:multilqt}
\end{align}
where the Schr\"{o}dinger potential $q$ is the same as before $q(\bx) = \ln \sigma (\bx)$.
The transformed boundary and initial conditions take the form \eqref{eq:in.3}--\eqref{eq:in.2}.

The entries of the matrix-valued multi-dimensional data $\bD_k \in \mathbb{R}^{m \times m}$, 
$k = 0, \ldots, 2n-1$, can be expressed in terms of the primary wave $P_s$ as 
\begin{equation}
(\bD_k)_{i,j} = \left< b_j, \cp_i(t_k,\cdot) \right>_{\frac{1}{c(\bx)}} = 
\int_\Omega \frac{d\bx}{c(\bx)} \cb_j(\bx) \cp_i(t_k, \bx), 
\quad i,j = 1,\ldots,m.
\label{eq:multidatab}
\end{equation}

%==================================================================================================
\subsection{Symmetrized data model, propagator and measurement function}
\label{sect:multisym}

The derivation of the multi-dimensional data model \eqref{eq:multidatab} follows closely the
derivation of its one-dimensional analogue \eqref{eq:1D21}. In order to write the data model in
the symmetrized form \eqref{eq:1D33} in one dimension we employed the transformation to
travel time coordinates \eqref{eq:1D23}. Unfortunately, such transformation is not available in
higher dimensions. Thus, we follow a different approach to obtain an analogue of \eqref{eq:1D33}.

Combining \eqref{eq:multidatab} with \eqref{eq:multipfrakcos} and \eqref{eq:multicpcu} we write
\begin{equation}
(\bD_k)_{i,j} = \int_{\Omega} \frac{d \bx}{c(\bx)} 
b_j(\bx) \sigma^{-1/2}(\bx) \cos(t_k \sqrt{A}) \sigma^{1/2}(\bx) b_i(\bx),
\end{equation}
where we assume for the remainder of this section $i,j = 1,\ldots,m$, and $k=0,\ldots,2n-1$.
From the definitions \eqref{eq:multilq}--\eqref{eq:multilqt} of $L_q$ and its adjoint it follows
\begin{equation}
A = \sigma^{1/2}(\bx) L_q L_q^T \sigma^{-1/2}(\bx),
\end{equation}
hence
\begin{equation}
(\bD_k)_{i,j} = \int_{\Omega} \frac{d \bx}{c(\bx)} b_j(\bx) 
\cos \Big( t_k \sqrt{L_q L_q^T} \Big) b_i(\bx),
\label{eq:multidatac}
\end{equation}
where we used the fact that analytic matrix functions commute with similarity transformations.
We employ another similarity transformation to rewrite \eqref{eq:multidatac} as
\begin{equation}
(\bD_k)_{i,j} = \int_{\Omega} d \bx \; b_j^c(\bx) 
\cos\Big(t_k \sqrt{c^{-1/2} L_q L_q^T c^{1/2}} \Big) b_i^c(\bx),
\label{eq:multidatad}
\end{equation}
where we introduced the rescaled sensor functions 
\begin{equation}
b^c_s (\bx) = \frac{b_s(\bx)}{\sqrt{c(\bx)}}, \quad s = 1,\ldots,m.
\end{equation}

In a slight abuse of notation, similarly to \eqref{eq:1D24}--\eqref{eq:1D25} we redefine 
\begin{align}
L_q   & = c^{1/2}(\bx) \left( - \nabla \cdot + \frac{1}{2} \nabla q(\bx) \; \cdot \right) c^{1/2}(\bx), 
\label{eq:multilqsym} \\
L_q^T & = c^{1/2}(\bx) \left( \nabla + \frac{1}{2} \nabla q(\bx) \right) c^{1/2}(\bx),
\label{eq:multilqtsym}
\end{align}
which are adjoint to each other with respect to the standard $L^2(\Omega)$ inner product.
With definitions \eqref{eq:multilqsym}--\eqref{eq:multilqtsym} at hand, we can define the 
propagator for the multi-dimensional problem
\begin{equation}
\msP = \cos \Big( \tau \sqrt{L_q L_q^T} \Big),
\label{eq:multiprop}
\end{equation}
exactly as in \eqref{eq:1D29}. Finally, we can write the data model \eqref{eq:multidatad}
in a symmetric form and introduce the matrix-valued measurement function 
$\bM_k(L_q L_q^T) \in \mathbb{R}^{m \times m}$ with components
\begin{equation}
(\bD_k)_{i,j} = [\bM_k (L_q L_q^T)]_{i,j} = 
\left< b_j^c(\bx), \mathcal{T}_k(\msP) b_i^c(\bx) \right>.
\end{equation}

Similarly to the one-dimensional case, the propagator $\msP$ can be used to define an
exact time stepping scheme for what we refer to as the symmetrized snapshots
\begin{equation}
\cp_{s,k}(\bx) = \mathcal{T}_k (\msP) \cb_s^c(\bx), \quad k=0,\ldots,2n-1, \quad s=1,\ldots,m.
\end{equation}
They satisfy the same second-order time stepping scheme \eqref{eq:1D39}:
\begin{equation}
\frac{\cp_{s, k+1} (\bx) - 2 \cp_{s, k} (\bx) + \cp_{s, k-1}(\bx)}{\tau^2} = 
-\xi(\msP) \cp_{s, k}(\bx), \quad k=0,\ldots,2n-1,
\label{eq:multitimestep}
\end{equation}
with initial conditions 
\begin{equation}
\cp_{s, 0} (\bx) = \cb^c_s(\bx), \quad \cp_{s, -1} (\bx) = \cp_{s, 1} (\bx) = \msP \cb^c_s (\bx),
\label{eq:multitsinit}
\end{equation}
where the affine function $\xi$ is given by \eqref{eq:defXi}. We can also consider the 
factorization \eqref{eq:1D41} of $\xi(\msP)$ in terms of the operator $\mathcal{L}_q$
given precisely by \eqref{eq:1D42}.

%==================================================================================================
\subsection{Multi-input, multi-output reduced order model}
\label{sect:mimorom}

The main difference between the cases of one and multiple dimensions is in the type of ROM 
that we use. While in the one-dimensional case a single-input, single output (SISO) 
projection ROM \eqref{eq:1D56p}, \eqref{eq:bb2} is employed to satisfy the data matching 
conditions \eqref{eq:1D50}, in the multi-dimensional case we need to consider a multi-input, 
multi-output (MIMO) ROM.

Similarly to section \eqref{sect:1D.2}, we introduce $\bA \in \mathbb{R}^{N \times N}$, 
a discretization of the operator \eqref{eq:multiA} on a very fine grid with a total of $N$ nodes. 
For simplicity, the grid is assumed uniform with cell size $h$ in all directions. Note that
the operator $A$ is related to $L_q$ and $L_q^T$ defined in 
\eqref{eq:multilqsym}--\eqref{eq:multilqtsym} as
\begin{equation}
A = [\sigma(\bx) c(\bx)]^{1/2} L_q L_q^T [\sigma(\bx) c(\bx)]^{-1/2}.
\end{equation}
Let $\boldsymbol \Sigma \in \mathbb{R}^{N \times N}$ and $\bC \in \mathbb{R}^{N \times N}$
be the diagonal matrices with entries given by $\sigma(\bx)$ and $c(\bx)$ respectively at $N$ 
fine grid nodes. Then we can set $\bL_q$, a fine grid approximation of $L_q$, to be a Cholesky 
factor of
\begin{equation}
{\boldsymbol \Sigma}^{-1/2} \bC^{-1/2} \bA {\boldsymbol \Sigma}^{1/2} \bC^{1/2} 
=  \bL_q \bL_q^T.
\end{equation}
We can argue that the discretized propagator $\bbP \in \mathbb{R}^{N \times N}$ is well 
approximated by \eqref{eq:approxP}.

When introducing the discretized symmetrized snapshots, it is convenient to arrange them into 
matrices $\bp_k \in \mathbb{R}^{N \times m}$, $k = 0,\ldots,2n-1$, with each column 
corresponding to a different sensor. Thus, they will satisfy a fine grid analogue of the
time-stepping scheme \eqref{eq:multitimestep} given by
\begin{equation}
\frac{\bp_{k+1} - 2 \bp_k + \bp_{k-1}}{\tau^2} = 
-\xi(\bbP) \bp_k, \quad k=0,\ldots,2n-1,
\label{eq:multitimesteppmat}
\end{equation}
with initial conditions
\begin{equation}
\bp_0 = \bb, \quad \bp_{-1} = \bp_1 = \bbP \bb.
\label{eq:multitsinitpmat}
\end{equation}
Here the sensor matrix $\bb \in \mathbb{R}^{N \times m}$ is defined columnwise
\begin{equation}
\bb = [\bb_1,\ldots,\bb_m],
\end{equation}
where the entries of each $\bb_s \in \mathbb{R}^N$, $s=1,\ldots,m$, are the values of the
corresponding rescaled sensor function $b_s^c(\bx)$ on the fine grid, multiplied by $h^{d/2}$.
Once the sensor matrix is introduced, we can write the discretized data model and measurement
functions
\begin{equation}
\bD_k = \bM_k(L_q L_q^T) \approx \bM_k (\bL_q \bL_q^T) = \bb^T \bp_k =
\bb^T \mathcal{T}_k (\bbP) \bb \in \mathbb{R}^{m \times m},
\label{eq:multidatadisc}
\end{equation}
for $k=0,\ldots,2n-1$. From \eqref{eq:multidatadisc} we obtain an analogue of \eqref{eq:bb}
relating the initial time data $\bD_0$ to the sensor matrix
\begin{equation}
\bD_0 = 
\begin{bmatrix} 
\left< b^c_1(\bx), b^c_1(\bx) \right> & \left< b^c_1(\bx), b^c_2(\bx) \right> & 
\ldots & \left< b^c_1(\bx), b^c_m(\bx) \right> \\
\left< b^c_2(\bx), b^c_1(\bx) \right> & \left< b^c_2(\bx), b^c_2(\bx) \right> & 
\ldots & \left< b^c_2(\bx), b^c_m(\bx) \right> \\
\vdots & \vdots & \ddots & \vdots \\
\left< b^c_m(\bx), b^c_1(\bx) \right> & \left< b^c_m(\bx), b^c_2(\bx) \right> & 
\ldots & \left< b^c_m(\bx), b^c_m(\bx) \right> 
\end{bmatrix} \approx 
\bb^T \bb,
\label{eq:multibb}
\end{equation}
and following the discussion in section \ref{sect:1D.2} we treat the approximate relations 
\eqref{eq:multidatadisc}--\eqref{eq:multibb} as equalities.

The MIMO ROM consists of the symmetric matrix $\tilde{\bbP} \in \mathbb{R}^{nm \times nm}$ and 
a matrix $\tilde \bb \in \mathbb{R}^{nm \times m}$ that satisfy the data matching conditions
\begin{equation}
\bD_k = \tilde \bb^T \mathcal{T}_k (\tilde{\bbP} ) \tilde \bb, 
\quad k = 0, \ldots, 2n-1.
\label{eq:multidatamatch}
\end{equation}
The matrix $\tilde{\bbP}$ has block tridiagonal structure with blocks of size $m \times m$,
while $\tilde \bb$ consists of all zeros except for the uppermost $m \times m$ block, 
and thus is given by
\begin{equation}
\tilde \bb = (\bD_0)^{1/2} \bE_1,
\end{equation}
where 
\begin{equation}
\bE_1 = \begin{bmatrix} 
\bI_m \\ {\boldsymbol 0}_m \\ \vdots \\ {\boldsymbol 0}_m 
\end{bmatrix} \in \mathbb{R}^{nm \times m},
\label{eq:e1mat}
\end{equation}
and ${\boldsymbol 0}_m \in \mathbb{R}^{m \times m}$ is the zero matrix.

%==================================================================================================
\subsection{Calculation of projection MIMO ROM}
\label{sect:mimoromcalc}

Similarly to its SISO counterpart, the MIMO ROM satisfying the data matching conditions 
\eqref{eq:multidatamatch} is given by the orthogonal projection of $\bbP$ on a certain subspace.
However, in the multi-dimensional case this is block Krylov subspace, spanned by the columns of
\begin{equation}
\bP = [\bp_0, \ldots, \bp_{n-1}] \in \mathbb{R}^{N \times nm}.
\end{equation}
We still denote by $\bV = [\bV_1,\ldots,\bV_n]$ the matrix containing the orthonormal basis 
for $\mbox{range}(\bP)$, however, in the multi-dimensional case $\bV \in \mathbb{R}^{N \times nm}$ 
with each $\bV_k$ being an $N \times m$ matrix. 

In order to compute the matrices $\bP^T \bP$ and $\bP^T \bbP \bP$ from the data we can still use 
the formulas \eqref{eq:MassM1} and \eqref{eq:Stiff2}, however, the indexing has to be understood 
blockwise, i.e. when we write
\begin{align}
\big(\bP^T \bP\big)_{i,j} & = \frac{1}{2} \Big( \bD_{i+j-2} + \bD_{|i-j|} \Big) 
\in \mathbb{R}^{m \times m}, \label{eq:multimassdata} \\
(\bP^T \bbP \bP)_{i,j} & = 
\frac{1}{4} \Big( \bD_{i+j-1} + \bD_{|j-i+1|} + \bD_{|j-i-1|} + \bD_{|j+i-3|} \Big) 
\in \mathbb{R}^{m \times m}, \label{eq:multistiffdata}
\end{align}
for $i,j = 1,\ldots,n$, we use notation $\big( \bP^T \bP \big)_{i,j}$ to refer to the 
$m \times m$ block of $\bP^T \bP \in \mathbb{R}^{nm \times nm}$ at the intersection of 
rows $(i-1)m+1,\ldots,im$ and columns $(j-1)m+1,\ldots,jm$. Hereafter we employ this 
notation for $\bP^T \bbP \bP \in \mathbb{R}^{nm \times nm}$ and all other block matrices 
with block size $m \times m$. Note that from \eqref{eq:multimassdata}--\eqref{eq:multistiffdata}
it follows that not only both $\bP^T \bP$ and $\bP^T \bbP \bP$ are symmetric, their 
individual blocks are symmetric as well.

For MIMO ROM we replace Cholesky factorization \eqref{eq:Chol1} with block Cholesky factorization.
Note that while the regular Cholesky factorization is defined uniquely, there is an ambiguity 
in defining block Cholesky factorization that comes from the computation of diagonal
blocks. The particular, they are uniquely defined up to an arbitrary rotation. The general form of the Cholesky factorization can be obtained by the
following algorithm.

\begin{alg}[Block Cholesky factorization]
\label{alg:blockhol}~\\
\textbf{Input:} Symmetric block matrix $\bX \in \mathbb{R}^{nm \times nm}$ with $m \times m$ blocks.

\vspace{0.05in} \noindent
To compute block Cholesky factorization of $\bX$ perform the following steps:

\vspace{0.05in} \noindent
For $k=0,1,\ldots,n-1:$
\begin{equation}
\bR_{k,k} = \bQ_k\Big( \bX_{k,k} - \sum_{i=0}^{k-1} \bR_{i,k}^T \bR_{i,k} \Big)^{1/2}
\end{equation}
where $\bQ_k\in \mathbb{R}^{m\times m}$ is an arbitrary orthogonal matrix.
~~~~~~~~~~~~~For $j=k+1,\ldots,n-1:$
\begin{equation}
\bR_{k,j} = \bR_{k,k}^{-1} \Big( \bX_{k,j} - \sum_{i=0}^{k-1} \bR_{i,k}^T \bR_{i,j} \Big).
\end{equation}

\vspace{0.05in} \noindent  \textbf{Output:} Block matrix $\bR \in \mathbb{R}^{nm \times nm}$
with $m \times m$ blocks, satisfying $\bX = \bR^T \bR$.
\end{alg}

Once the block Cholesky factor $\bR$ is computed, the MIMO ROM matrix $\tilde{\bbP}$ is given
by \eqref{eq:1D56p}. Clearly, if $\bQ_k={\itbf I}_m, ~k=1,\ldots, n$ then the diagonal blocks $\bR_{k,k},~k=1,\ldots, n$ are symmetric.  We denote the corresponding MIMO ROM matrix as $\tilde{\bbP}^{{\itbf I}}$. 

%==================================================================================================
\subsection{Factorization of MIMO ROM and data to Born transform}
\label{sect:mimoromfactor}

As mentioned in section \ref{sect:mimoromcalc}, block Cholesky factorization is not uniquely
defined. For non-trivial orthogonal matrices $\bQ_k, ~k=1,\ldots, n$, the corresponding MIMO ROM matrix $\tilde{\bbP}^{\bQ}$ is given by $\bQ\tilde{\bbP}^{{\itbf I}}\bQ^T$ where $\bQ$ is block-diagonal matrix with orthogonal blocks $\bQ_k, ~k=1,\ldots, n$. However, the block bidiagonal factor  $\tbL_q$ in \eqref{eq:Chol} has to be consistent with the matrix analogue of the recursion \eqref{eq:O1}--\eqref{eq:O3p} for computing primary and dual orthogonalized block snapshots $\overline{\bp}_{j}\in \mathbb{R}^{N \times m}$ and $\overline{\bcu}_{j}\in \mathbb{R}^{N \times m}, ~j=1,\ldots,n$, respectively, 
\begin{align}
\gamma^{-1}_j\left(\overline{\bp}_{j+1} - \overline{\bp}_{j}\right) = - \cbL_q
\overline{\bcu}_j, \quad \hat \gamma^{-1}_j\left(\overline{\bcu}_{j} -
  \overline{\bcu}_{j-1}\right) = \cbL_q^T \overline{\bp}_j,
\label{eq:O1b}
\end{align}
for $j \ge 1$, with initial conditions 
\begin{equation}
\overline{\bp}_{1} = \bb, \quad \overline{\bcu}_{0} = 0,
\label{eq:O2b}
\end{equation}
and coefficients
% \footnote{Recall the Liouville transformation
%  \eqref{eq:1D17}. The snapshots of $\mathfrak{p}$ and $\mathfrak{u}$
%  in that formula are the ones orthogonalized in
%  \cite{druskin2016direct}. If we denote those snapshots by
%  $\overline{\mathfrak{p}}_j$ and $\overline{\mathfrak{u}}_j$, since
%  $\|\overline{\mathfrak{u}}_j\|^2_{\sigma} = \|\overline \bcu_j\|^2$
%  and $\|\overline{\mathfrak{p}}_j\|^2_{1/\sigma} = \|\overline
%  \bp_j\|^2$, we should have the same coefficients $\gamma_j$ and
%  $\hat \gamma_j$ in \eqref{eq:O1}.}
\begin{equation}
0< \gamma_j = \gamma^T_j=\|\overline{\bcu}_j\|^{-2}\in \mathbb{R}^{m \times m}, \quad 
0< \hat \gamma_j = \hat \gamma^T_j = \|\overline{\bp}_j\|^{-2}\in \mathbb{R}^{m \times m}, \quad j = 1, \ldots, n.
\label{eq:O3b}
\end{equation}
\begin{align}
(\tbL_q)_{j,j} &= -\sqrt{\hat \gamma^{-1}_j}\sqrt{\gamma^{-1}_j }, \quad j = 1,
  \ldots, n, \nonumber \\ 
(\tbL_q)_{j+1,j} &= \sqrt{\hat
    \gamma^{-1}_{j+1}}\sqrt{\gamma^{-1}_{j}}, \quad j = 1, \ldots, n-1.
\label{eq:O3pb}
\end{align}
Below we shall single out such matrix $\bQ$ that the factorization of 
\begin{equation}
\label{eq:romeqchol}
\bQ\tilde{\bbP}^{{\itbf I}}\bQ^T=\tbL_q\tbL^T_q
\end{equation} corresponds to $\tbL_q$ of the form \eqref{eq:O3pb} with symmetric positive $\gamma_j$ and $\hat \gamma_j, ~j=1,\ldots, n$. Denote the diagonal and the off-diagonal blocks of $\tilde{\bbP}^{{\itbf I}}$ as $\alpha_i\in\mathbb{R}^{m \times m}, i=1,\ldots,n$ and $-\beta_i\in\mathbb{R}^{m \times m}, i=2,\ldots,n$, respectively. By definition, 
\begin{equation}
\label{eq:gammahat1}
\hat\gamma_1=\|\ \bb\|^{-2}. 
\end{equation}

The remaining matrix coefficients $\gamma_j$ and $\hat\gamma_j$ are obtained from \eqref{eq:romeqchol} blockwise. In particular, from the first diagonal block we obtain that $\sqrt{\hat \gamma^{-1}_1}\gamma^{-1}_1\sqrt{\hat \gamma^{-1}_1}=\bQ_{1}\alpha_1\bQ^T_1$, or, equivalently,   
\begin{equation}
\label{eq:gamma1}
\gamma_1=\left(\sqrt{\hat \gamma_1}\bQ_1\alpha_1\bQ^T_1\sqrt{\hat \gamma_1}\right)^{-1}. 
\end{equation}
Clearly, $\gamma_1=\gamma^T_1$ for any matrix $\bQ_1$, so for simplicity we set $\bQ_1={\itbf I}_m$. Then, from off-diagonal blocks for $1\le i\le n-1$ we have $\sqrt{\hat \gamma^{-1}_i}\gamma^{-1}_i\sqrt{\hat \gamma^{-1}_{i+1}}=\bQ_{i}\beta_{i+1}\bQ^T_{i+1}$. Hence, $\sqrt{\hat \gamma^{-1}_{i+1}}\bQ_{i+1}=\gamma_i\sqrt{\hat \gamma_i}\bQ_{i}\beta_{i+1}$, or, in other words, that a pair of matrices $\left(\sqrt{\hat \gamma^{-1}_{i+1}},\bQ_{i+1}\right)$ is a (left) polar decomposition of
\begin{equation}
\label{eq:poldecmtr}
\bM_i=\gamma_i\sqrt{\hat \gamma_i}\bQ_{i}\beta_{i+1}.
\end{equation}
Its solution is 
\begin{align}
\label{eq:gammahatip1}
\hat \gamma_{i+1}=\left(\bM_i\bM^T_i\right)^{-1}
\\
\bQ_{i+1}=\sqrt{\hat \gamma_{i+1}}\bM_i.
\label{eq:poldecorth}
\end{align}
Finally, considering diagonal blocks for $1\le i\le n-1$, we obtain $\sqrt{\hat \gamma^{-1}_{i+1}}\left(\gamma^{-1}_i+\gamma^{-1}_{i+1}\right)\sqrt{\hat \gamma^{-1}_{i+1}}=\bQ_{i+1}\alpha_{i+1}\bQ^T_{i+1}$, or, consequently, 
\begin{equation}
\label{eq:gammaip1}
\gamma_{i+1}=\left(\sqrt{\hat \gamma_{i+1}}\bQ_{i+1}\alpha_{i+1}\bQ^T_{i+1}\sqrt{\hat \gamma_{i+1}}-\gamma^{-1}_i\right)^{-1}.
\end{equation}

So, we summarize the algorithm to compute $\tbL_q$ consistent with recursion \eqref{eq:O1b}--\eqref{eq:O3pb} as follows
\begin{alg}[Computation of $\tbL_q$]
\label{alg:blockholwgm}~\\
\textbf{Input:} Block tridiagonal matrix $\tilde{\bbP}^{{\itbf I}} \in \mathbb{R}^{nm \times nm}$ with $m \times m$ blocks and the norm $\|\ \bb\|$.

\vspace{0.05in} \noindent
To find such $\bQ$ that the block Cholesky factorization $\tbL_q\tbL^T_q$ of $\tilde{\bbP}^{\bQ}$ has factors $\tbL_q$ in the form \eqref{eq:O3pb}, perform the following steps:
\begin{enumerate}
\item Compute $\hat\gamma_1$ via \eqref{eq:gammahat1}
\item Compute $\gamma_1$ via \eqref{eq:gamma1} for arbitrary $\bQ_1$ (for simplicity, we set $\bQ_1={\itbf I}_m$)
\vspace{0.05in} \noindent
\item For $i=1,\ldots,n-1:$
\begin{enumerate}
\item Compute $\hat \gamma_{i+1}$ and $\bQ_{i+1}$ via \eqref{eq:gammahatip1} and \eqref{eq:poldecorth} for $\bM_i$ given by \eqref{eq:poldecmtr}
\item Compute $\gamma_{i+1}$ via \eqref{eq:gammaip1}
\end{enumerate}

\vspace{0.05in} \noindent
\item Compute $\tbL_q$ via \eqref{eq:O3pb}
\end{enumerate}
\textbf{Output:} Block diagonal orthogonal matrix $\bQ$, the block tridiagonal matrix $\tilde{\bbP}^{\bQ}=\bQ\tilde{\bbP}^{{\itbf I}}\bQ^T$ and its block lower bidiagonal factor $\tbL_q$ consistent with \eqref{eq:O3pb}
\end{alg}


After the  factor $\tbL_q$ is found, the data to Born transform is 
computed using Algorithms \ref{eq:algo1} and \ref{alg:chain}, with $\bb_0$ and ${\bf e}_1=\left({\itbf I}_m,0,\ldots,0\right)$ being tall matrix of input vectors and block first unit vector. 









